Empirical Relevance of Ambiguity in First Price Auction Models

We study the identification and estimation of first-price auction models where bidders have ambiguity about the valuation distribution and their preferences are represented by maxmin expected utility. When entry is exogenous, the distribution and ambiguity structure are nonparametrically identified, separately from risk aversion (CRRA). We propose a flexible Bayesian method based on Bernstein polynomials. Monte Carlo experiments show that our method estimates parameters precisely, and chooses reserve prices with (nearly) optimal revenues, whether there is ambiguity or not. Furthermore, if the model is misspecified -- incorrectly assuming no ambiguity among bidders -- it may induce estimation bias with a substantial revenue loss.

==> options-kam.tex <==
\usepackage{xifthen}
	\newboolean{historynotate}
					\setboolean{historynotate}{false}


\usepackage{setspace}
\usepackage{boxedminipage}
\usepackage{color}
\usepackage{relsize}
\usepackage[greek,english]{babel}

\ifx\pdfoutput\undefined
	\usepackage{graphicx}
\else
	\usepackage[pdftex]{graphicx}
\fi


% TIKZ plotting
\usepackage{tikz}
%\usetikzlibrary{arrows, calc, shapes}
%\tikzset{
%	%Define standard arrow tip
%	>=stealth',
%	%Define style for different line styles
%	help lines/.style={dashed, thick},
%	axis/.style={<->},
%	important line/.style={thick},
%	connection/.style={thick, dotted},
%}

\usepackage{epstopdf}
\usepackage{url}
\usepackage{bm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{array}
\usepackage{mathrsfs}
\usepackage[multiple]{footmisc}
\usepackage[para]{manyfoot}
\usepackage{subfig}
\usepackage{dcolumn}

% FONT OPTIONS
\usepackage{mathpazo}  % Global font change to: palatino, including math (where possible)
					% Default is CM Roman in LaTeX
					% Junsang - This is what you want - the Doepke fonts?
					
%\usepackage[T1]{fontenc}
%\usepackage[light,math]{anttor}

 \makeatletter
 \let\NAT@parse\undefined
 \makeatother
 \usepackage[square]{natbib}

% CUSTOM COLORS
\definecolor{sangre}{rgb}{0.6,0.18,0.19}
\definecolor{dullmagenta}{rgb}{0.4,0,0.4}
\definecolor{darkblue}{rgb}{0,0,0.6}


\ifx\pdfoutput\undefined
\usepackage[backref=none,hypertex,colorlinks,urlcolor = darkblue,citecolor = sangre,linkcolor=blue]{hyperref}
\else
\usepackage[backref=page,pdftex,hypertexnames=false,colorlinks,urlcolor = darkblue,citecolor =  sangre,linkcolor=blue]{hyperref}
\fi

% SPACING AND MARGINS
\vspace{\bigskipamount}
\renewcommand{\baselinestretch}{1.3}
\usepackage[left=3.5cm,right=3.5cm,top=4cm,bottom=4cm]{geometry}

% THEOREM ENVIRONMENTS
\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{assumption}{Assumption}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{result}[theorem]{Result}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}

%\newenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

% CUSTOM SHORTCUT MATH / PROGRAMMING COMMANDS

	% Figure/font sizes
	\newcommand{\figurewidthscale}{0.4}
	\newcommand{\prooffontsize}{\relsize{-1}}
	
	% Math shortcuts
	\newcommand{\mb}{\mathbf}
	\newcommand{\mbb}{\mathbb}
	\newcommand{\mcl}{\mathcal}
	\newcommand{\C}{\mb{C}}
	\newcommand{\R}{\mbb{R}}
	\newcommand{\N}{\mbb{N}}
	\newcommand{\Z}{\mbb{Z}}
	\newcommand{\E}{\mbb{E}}
	\newcommand{\EE}{\widetilde{\mbb{E}}}
	\newcommand{\diff}{\text{d}}
	\newcommand{\hz}{\hat{z}}
	
	% Typical macro paper notations:
	\newcommand{\kv}{\mb{k}}
	\newcommand{\bv}{b}
	\newcommand{\Kv}{\mb{K}}
	\newcommand{\Bv}{B}
	\newcommand{\sv}{\mb{s}}
	\newcommand{\zv}{\mb{z}}
	\newcommand{\ev}{\mb{v}}
	\newcommand{\av}{\mb{a}}
	\newcommand{\pv}{\mb{p}}
	
	% Begin/End equation environment
	\def\beq{\begin{equation}}
	\def\eeq{\end{equation}}

	% Program Names:
	\def\matlab{{\scshape\texttt{Matlab}}}
	\def\octave{{\scshape\texttt{Octave}}}
	\def\python{{\scshape\texttt{Python}}}
	\def\Rsoftware{{\scshape\texttt{R}}}
	
	% Underscore:
	\def\us{\char`\_}
	
	\ifthenelse{\boolean{historynotate}}{
		% Use ''t-history notation'':
		\newcommand{\thist}{h^{t}}
		\newcommand{\pthist}{\left(h^{t}\right)}
		\newcommand{\shist}{h^{s}}
		\newcommand{\pshist}{(h^{s})}
		\newcommand{\thistplus}{h^{t+1}}
		\newcommand{\pthistlag}{(h^{t-1})}
		\newcommand{\pthistplus}{\left(h^{t+1}\right)}
		\newcommand{\nexthist}{(z_{t+1},\thist)}
		\newcommand{\nexthistplustau}{h^{t+\tau}}
		\newcommand{\pnexthistplustau}{(h^{t+\tau})}
		\newcommand{\nexttauhist}{(z_{t+\tau},\thist)}
		\newcommand{\icomma}{i,}
	}
	{	
		% Or don't use ''t-history notation'': 
		\newcommand{\thist}{}
		\newcommand{\pthist}{}
		\newcommand{\shist}{}
		\newcommand{\pshist}{}
		\newcommand{\thistplus}{}
		\newcommand{\thistlag}{}
		\newcommand{\pthistplus}{}
		\newcommand{\nexthist}{}
		\newcommand{\nexthistplustau}{}
		\newcommand{\pnexthistplustau}{}
		\newcommand{\nexttauhist}{}
		\newcommand{\icomma}{i}
	}
	
	% List shortcuts
	\newcommand{\pse}{\pause}
	\newcommand{\bol}{\begin{enumerate}}
	\newcommand{\eol}{\end{enumerate}}
	\newcommand{\bul}{\begin{itemize}}
	\newcommand{\eul}{\end{itemize}}
	\newcommand{\li}{\item}
 
 
 % Footnote misc.
 \DeclareNewFootnote[para]{B}[alph]
 
  % Custom To Do Notes

\newcommand{\smalltodo}[2][]{\todo[caption={#2}, #1]{\begin{spacing}{0.8}#2\end{spacing}}} % Tighten spacing

% Ordered To Do Note list
	\newcounter{todocounter}
	\newcommand{\todonum}[2][]
	{\stepcounter{todocounter}\todo[#1]{\thetodocounter: #2}}

